Three subpopulations of binary black holes in mass, spin magnitudes and tilts following GWTC-5

The mass and spin distributions of merging binary black holes offer clues to their formation pathways, which remain uncertain. In this work, we model the population of binary black holes using generic subpopulations with distinct mass-ratio, spin-magnitude, and spin-tilt distributions, whose relative contributions vary with primary mass. Using the 259 binary black holes in the fifth LIGO-Virgo-KAGRA catalog (GWTC-5), we resolve three subpopulations with low, medium, and high spins. The low-spin population dominates for primary masses near $35 M_\odot$, contributes roughly half of the binaries for primary masses of $10 M_\odot$, and favors nearly equal mass ratios overall; its spins are consistent with both black holes having negligible spin, with a log Bayes factor of $\log_{10}B =6.1^{+0.2}_{-0.3}$ in favor of vanishing spins. The medium-spin population accounts for the other half of the population around primary masses of $10 M_\odot$ and favors spin magnitudes $\chi_i \approx 0.2$ for both components, preferentially aligned orientations, and comparable mass ratios. The high-spin population dominates above primary masses of $60 M_\odot$ and also contributes at lower masses $\sim 20 M_\odot$; it favors a rapidly spinning primary ($\chi_1 \approx 0.7$), a broad range of secondary spins, widely distributed spin orientations, and a broad mass-ratio distribution. Allowing for a fourth subpopulation yields no distinct additional mass-ratio or spin distribution, as it becomes degenerate with existing features. To resolve highly concentrated features in spin, we control the variance of standard Monte Carlo likelihood estimators using truncated Gaussian mixture models. Taken together, our results add to a growing body of evidence for substructure in the population of LIGO-Virgo-KAGRA black holes, providing further clues to uncover their formation histories.

==> figures/FiducialModel/macros.tex <==
% Generated from macros.json by scripts/json2tex.py -- do not edit.
\JSONSetValue{mass_breakpoints[0]}{13^{+5}_{-3}}
\JSONSetValue{mass_breakpoints[1]}{18^{+12}_{-7}}
\JSONSetValue{mass_breakpoints[2]}{40^{+10}_{-10}}
\JSONSetValue{mass_breakpoints[3]}{60^{+40}_{-20}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.A}{0.5^{+0.2}_{-0.1}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.B}{0.4^{+0.2}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.C}{0.05^{+0.10}_{-0.05}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.A}{0.8^{+0.1}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.B}{0.05^{+0.26}_{-0.05}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.C}{0.13^{+0.11}_{-0.09}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.A}{0.8^{+0.1}_{-0.1}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.B}{0.02^{+0.05}_{-0.02}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.C}{0.13^{+0.12}_{-0.11}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.A}{0.2^{+0.4}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.B}{0.06^{+0.14}_{-0.06}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.C}{0.68^{+0.29}_{-0.37}}
\JSONSetValue{mass_ranges.Flat[0]}{<13^{+5}_{-3}}
\JSONSetValue{mass_ranges.Flat[1]}{18^{+12}_{-7} - 40^{+10}_{-10}}
\JSONSetValue{mass_ranges.Flat[2]}{>60^{+40}_{-20}}
\JSONSetValue{mass_ranges.Transition[0]}{13^{+5}_{-3} - 18^{+12}_{-7}}
\JSONSetValue{mass_ranges.Transition[1]}{40^{+10}_{-10} - 60^{+40}_{-20}}
%\JSONSetValue{subpop_hyperposteriors.a.mu.chi_1}{0.017^{+0.023}_{-0.017}}
\JSONSetValue{subpop_hyperposteriors.a.mu.chi_1}{0.02^{+0.02}_{-0.02}}
%\JSONSetValue{subpop_hyperposteriors.a.mu.chi_2}{0.013^{+0.022}_{-0.013}}
\JSONSetValue{subpop_hyperposteriors.a.mu.chi_2}{0.01^{+0.03}_{-0.01}}
\JSONSetValue{subpop_hyperposteriors.a.mu.cos_tilt_1}{-0.03^{+0.06}_{-0.06}}
\JSONSetValue{subpop_hyperposteriors.a.mu.cos_tilt_2}{-0.01^{+0.07}_{-0.07}}
\JSONSetValue{subpop_hyperposteriors.a.mu.mass_ratio}{1.12^{+0.08}_{-0.12}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.chi_1}{0.02^{+0.02}_{-0.02}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.chi_2}{0.01^{+0.02}_{-0.01}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.cos_tilt_1}{0.02^{+0.03}_{-0.02}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.cos_tilt_2}{0.02^{+0.04}_{-0.02}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.mass_ratio}{0.29^{+0.08}_{-0.09}}
\JSONSetValue{subpop_hyperposteriors.a.rho}{-0.2^{+0.8}_{-0.7}}
\JSONSetValue{subpop_hyperposteriors.b.mu.chi_1}{0.17^{+0.06}_{-0.06}}
\JSONSetValue{subpop_hyperposteriors.b.mu.chi_2}{0.15^{+0.08}_{-0.13}}
\JSONSetValue{subpop_hyperposteriors.b.mu.cos_tilt_1}{0.7^{+0.3}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.b.mu.cos_tilt_2}{0.6^{+0.3}_{-0.3}}
\JSONSetValue{subpop_hyperposteriors.b.mu.mass_ratio}{1.1^{+0.1}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.chi_1}{0.03^{+0.04}_{-0.03}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.chi_2}{0.05^{+0.09}_{-0.05}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.cos_tilt_1}{0.1^{+0.3}_{-0.1}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.cos_tilt_2}{0.1^{+0.3}_{-0.1}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.mass_ratio}{0.3^{+0.3}_{-0.1}}
\JSONSetValue{subpop_hyperposteriors.b.rho}{-0.3^{+0.9}_{-0.6}}
\JSONSetValue{subpop_hyperposteriors.c.mu.chi_1}{0.8^{+0.2}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.c.mu.chi_2}{0.6^{+0.4}_{-0.4}}
\JSONSetValue{subpop_hyperposteriors.c.mu.cos_tilt_1}{0.6^{+0.4}_{-1.1}}
\JSONSetValue{subpop_hyperposteriors.c.mu.cos_tilt_2}{0.2^{+0.8}_{-0.9}}
\JSONSetValue{subpop_hyperposteriors.c.mu.mass_ratio}{0.6^{+0.4}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.chi_1}{0.2^{+0.5}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.chi_2}{0.6^{+0.4}_{-0.4}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.cos_tilt_1}{1.0^{+0.8}_{-1.0}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.cos_tilt_2}{1.0^{+0.9}_{-0.8}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.mass_ratio}{0.5^{+0.3}_{-0.3}}
\JSONSetValue{subpop_hyperposteriors.c.rho}{-0.0^{+0.8}_{-0.8}}
\JSONSetValue{subpop_ppds.a.chi_1}{0.02^{+0.03}_{-0.02}}
\JSONSetValue{subpop_ppds.a.chi_2}{0.02^{+0.03}_{-0.02}}
\JSONSetValue{subpop_ppds.a.cos_tilt_1}{-0.03^{+0.08}_{-0.08}}
\JSONSetValue{subpop_ppds.a.cos_tilt_2}{-0.01^{+0.10}_{-0.09}}
\JSONSetValue{subpop_ppds.a.mass_ratio}{0.8^{+0.2}_{-0.3}}
\JSONSetValue{subpop_ppds.b.chi_1}{0.16^{+0.08}_{-0.08}}
\JSONSetValue{subpop_ppds.b.chi_2}{0.2^{+0.1}_{-0.1}}
\JSONSetValue{subpop_ppds.b.cos_tilt_1}{0.7^{+0.3}_{-0.4}}
\JSONSetValue{subpop_ppds.b.cos_tilt_2}{0.6^{+0.4}_{-0.4}}
\JSONSetValue{subpop_ppds.b.mass_ratio}{0.8^{+0.2}_{-0.4}}
\JSONSetValue{subpop_ppds.c.chi_1}{0.7^{+0.3}_{-0.4}}
\JSONSetValue{subpop_ppds.c.chi_2}{0.6^{+0.4}_{-0.4}}
\JSONSetValue{subpop_ppds.c.cos_tilt_1}{0.2^{+0.8}_{-0.9}}
\JSONSetValue{subpop_ppds.c.cos_tilt_2}{0.1^{+0.9}_{-0.8}}
\JSONSetValue{subpop_ppds.c.mass_ratio}{0.5^{+0.4}_{-0.4}}
\JSONSetValue{log_bayes_factors.in_favor_of_component_a_being_zero_spin}{6.1^{+0.2}_{-0.3}}


==> figures/FourRegimes/macros.tex <==
% Generated from macros.json by scripts/json2tex.py -- do not edit.
\JSONSetValue{mass_breakpoints[0]}{13^{+7}_{-3}}
\JSONSetValue{mass_breakpoints[1]}{20^{+10}_{-9}}
\JSONSetValue{mass_breakpoints[2]}{40^{+10}_{-10}}
\JSONSetValue{mass_breakpoints[3]}{60^{+30}_{-20}}
\JSONSetValue{mass_breakpoints[4]}{110^{+60}_{-60}}
\JSONSetValue{mass_breakpoints[5]}{160^{+40}_{-60}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.A}{0.5^{+0.1}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.B}{0.4^{+0.2}_{-0.1}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.C}{0.06^{+0.09}_{-0.06}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.spinning}{0.48^{+0.17}_{-0.15}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.fast}{0.057^{+0.094}_{-0.056}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.A}{0.7^{+0.2}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.B}{0.10^{+0.23}_{-0.10}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.C}{0.12^{+0.11}_{-0.08}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.spinning}{0.26^{+0.23}_{-0.16}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.fast}{0.120^{+0.114}_{-0.085}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.A}{0.8^{+0.1}_{-0.1}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.B}{0.03^{+0.05}_{-0.02}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.C}{0.112^{+0.104}_{-0.099}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.spinning}{0.15^{+0.11}_{-0.12}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.fast}{0.112^{+0.104}_{-0.099}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.A}{0.2^{+0.3}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.B}{0.07^{+0.14}_{-0.06}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.C}{0.70^{+0.26}_{-0.31}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.spinning}{0.80^{+0.20}_{-0.29}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.fast}{0.70^{+0.26}_{-0.31}}
\JSONSetValue{mass_ranges.Flat[0]}{<13^{+7}_{-3}}
\JSONSetValue{mass_ranges.Flat[1]}{20^{+10}_{-9} - 40^{+10}_{-10}}
\JSONSetValue{mass_ranges.Flat[2]}{60^{+30}_{-20} - 110^{+60}_{-60}}
\JSONSetValue{mass_ranges.Flat[3]}{>160^{+40}_{-60}}
\JSONSetValue{mass_ranges.Transition[0]}{13^{+7}_{-3} - 20^{+10}_{-9}}
\JSONSetValue{mass_ranges.Transition[1]}{40^{+10}_{-10} - 60^{+30}_{-20}}
\JSONSetValue{mass_ranges.Transition[2]}{110^{+60}_{-60} - 160^{+40}_{-60}}
\JSONSetValue{subpop_hyperposteriors.a.mu.chi_1}{0.015^{+0.022}_{-0.015}}
\JSONSetValue{subpop_hyperposteriors.a.mu.chi_2}{0.014^{+0.026}_{-0.014}}
\JSONSetValue{subpop_hyperposteriors.a.mu.cos_tilt_1}{-0.04^{+0.06}_{-0.05}}
\JSONSetValue{subpop_hyperposteriors.a.mu.cos_tilt_2}{-0.00^{+0.07}_{-0.06}}
\JSONSetValue{subpop_hyperposteriors.a.mu.mass_ratio}{1.11^{+0.09}_{-0.14}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.chi_1}{0.01^{+0.02}_{-0.01}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.chi_2}{0.01^{+0.03}_{-0.01}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.cos_tilt_1}{0.02^{+0.03}_{-0.02}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.cos_tilt_2}{0.03^{+0.03}_{-0.03}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.mass_ratio}{0.30^{+0.08}_{-0.10}}
\JSONSetValue{subpop_hyperposteriors.a.rho}{-0.1^{+0.8}_{-0.8}}
\JSONSetValue{subpop_hyperposteriors.b.mu.chi_1}{0.16^{+0.07}_{-0.06}}
\JSONSetValue{subpop_hyperposteriors.b.mu.chi_2}{0.2^{+0.1}_{-0.1}}
\JSONSetValue{subpop_hyperposteriors.b.mu.cos_tilt_1}{0.6^{+0.4}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.b.mu.cos_tilt_2}{0.7^{+0.3}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.b.mu.mass_ratio}{1.0^{+0.2}_{-0.3}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.chi_1}{0.03^{+0.06}_{-0.03}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.chi_2}{0.05^{+0.09}_{-0.05}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.cos_tilt_1}{0.1^{+0.3}_{-0.1}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.cos_tilt_2}{0.1^{+0.3}_{-0.1}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.mass_ratio}{0.4^{+0.3}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.b.rho}{-0.4^{+1.0}_{-0.5}}
\JSONSetValue{subpop_hyperposteriors.c.mu.chi_1}{0.8^{+0.2}_{-0.1}}
\JSONSetValue{subpop_hyperposteriors.c.mu.chi_2}{0.6^{+0.4}_{-0.5}}
\JSONSetValue{subpop_hyperposteriors.c.mu.cos_tilt_1}{0.5^{+0.5}_{-1.1}}
\JSONSetValue{subpop_hyperposteriors.c.mu.cos_tilt_2}{0.2^{+0.8}_{-0.9}}
\JSONSetValue{subpop_hyperposteriors.c.mu.mass_ratio}{0.6^{+0.4}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.chi_1}{0.1^{+0.4}_{-0.1}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.chi_2}{0.6^{+0.4}_{-0.4}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.cos_tilt_1}{1.0^{+0.8}_{-1.0}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.cos_tilt_2}{1.0^{+0.9}_{-0.8}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.mass_ratio}{0.5^{+0.3}_{-0.3}}
\JSONSetValue{subpop_hyperposteriors.c.rho}{0.0^{+0.9}_{-0.7}}
\JSONSetValue{subpop_ppds.a.chi_1}{0.02^{+0.03}_{-0.02}}
\JSONSetValue{subpop_ppds.a.chi_2}{0.02^{+0.04}_{-0.02}}
\JSONSetValue{subpop_ppds.a.cos_tilt_1}{-0.04^{+0.08}_{-0.08}}
\JSONSetValue{subpop_ppds.a.cos_tilt_2}{-0.00^{+0.09}_{-0.09}}
\JSONSetValue{subpop_ppds.a.mass_ratio}{0.8^{+0.2}_{-0.3}}
\JSONSetValue{subpop_ppds.b.chi_1}{0.16^{+0.09}_{-0.09}}
\JSONSetValue{subpop_ppds.b.chi_2}{0.2^{+0.1}_{-0.1}}
\JSONSetValue{subpop_ppds.b.cos_tilt_1}{0.6^{+0.4}_{-0.4}}
\JSONSetValue{subpop_ppds.b.cos_tilt_2}{0.6^{+0.4}_{-0.4}}
\JSONSetValue{subpop_ppds.b.mass_ratio}{0.7^{+0.3}_{-0.4}}
\JSONSetValue{subpop_ppds.c.chi_1}{0.8^{+0.2}_{-0.3}}
\JSONSetValue{subpop_ppds.c.chi_2}{0.5^{+0.4}_{-0.4}}
\JSONSetValue{subpop_ppds.c.cos_tilt_1}{0.1^{+0.9}_{-0.9}}
\JSONSetValue{subpop_ppds.c.cos_tilt_2}{0.1^{+0.9}_{-0.9}}
\JSONSetValue{subpop_ppds.c.mass_ratio}{0.6^{+0.4}_{-0.4}}
\JSONSetValue{log_bayes_factors.in_favor_of_component_a_being_zero_spin}{6.5^{+0.3}_{-0.3}}


==> figures/broad_q/macros.tex <==
\JSONSetValue{mass_breakpoints[0]}{12^{+7}_{-2}}
\JSONSetValue{mass_breakpoints[1]}{17^{+13}_{-6}}
\JSONSetValue{mass_breakpoints[2]}{40^{+50}_{-20}}
\JSONSetValue{mass_breakpoints[3]}{60^{+90}_{-20}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.A}{0.5^{+0.2}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.B}{0.4^{+0.2}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.C}{0.06^{+0.10}_{-0.06}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.spinning}{0.46^{+0.17}_{-0.18}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_10.fast}{0.056^{+0.105}_{-0.056}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.A}{0.7^{+0.2}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.B}{0.02^{+0.22}_{-0.02}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.C}{0.2^{+0.2}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.spinning}{0.29^{+0.18}_{-0.18}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_20.fast}{0.21^{+0.20}_{-0.16}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.A}{0.7^{+0.2}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.B}{0.02^{+0.07}_{-0.02}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.C}{0.22^{+0.20}_{-0.18}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.spinning}{0.26^{+0.19}_{-0.18}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_35.fast}{0.22^{+0.20}_{-0.18}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.A}{0.2^{+0.4}_{-0.2}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.B}{0.04^{+0.12}_{-0.04}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.C}{0.72^{+0.26}_{-0.36}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.spinning}{0.80^{+0.20}_{-0.38}}
\JSONSetValue{fraction_at_masses.fraction_at_mass_60.fast}{0.72^{+0.26}_{-0.36}}
\JSONSetValue{mass_ranges.Flat[0]}{<12^{+7}_{-2}}
\JSONSetValue{mass_ranges.Flat[1]}{17^{+13}_{-6} - 40^{+50}_{-20}}
\JSONSetValue{mass_ranges.Flat[2]}{>60^{+90}_{-20}}
\JSONSetValue{mass_ranges.Transition[0]}{12^{+7}_{-2} - 17^{+13}_{-6}}
\JSONSetValue{mass_ranges.Transition[1]}{40^{+50}_{-20} - 60^{+90}_{-20}}
\JSONSetValue{subpop_hyperposteriors.a.mu.chi_1}{0.018^{+0.024}_{-0.018}}
\JSONSetValue{subpop_hyperposteriors.a.mu.chi_2}{0.013^{+0.022}_{-0.013}}
\JSONSetValue{subpop_hyperposteriors.a.mu.cos_tilt_1}{-0.03^{+0.06}_{-0.06}}
\JSONSetValue{subpop_hyperposteriors.a.mu.cos_tilt_2}{-0.02^{+0.07}_{-0.07}}
\JSONSetValue{subpop_hyperposteriors.a.mu.mass_ratio}{1.12^{+0.08}_{-0.11}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.chi_1}{0.02^{+0.02}_{-0.02}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.chi_2}{0.01^{+0.02}_{-0.01}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.cos_tilt_1}{0.02^{+0.03}_{-0.02}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.cos_tilt_2}{0.03^{+0.04}_{-0.03}}
\JSONSetValue{subpop_hyperposteriors.a.sigma.mass_ratio}{0.2^{+0.1}_{-0.1}}
\JSONSetValue{subpop_hyperposteriors.a.rho}{-0.2^{+0.8}_{-0.7}}
\JSONSetValue{subpop_hyperposteriors.b.mu.chi_1}{0.16^{+0.07}_{-0.07}}
\JSONSetValue{subpop_hyperposteriors.b.mu.chi_2}{0.14^{+0.09}_{-0.13}}
\JSONSetValue{subpop_hyperposteriors.b.mu.cos_tilt_1}{0.7^{+0.3}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.b.mu.cos_tilt_2}{0.7^{+0.3}_{-0.3}}
\JSONSetValue{subpop_hyperposteriors.b.mu.mass_ratio}{1.0^{+0.2}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.chi_1}{0.03^{+0.06}_{-0.03}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.chi_2}{0.06^{+0.10}_{-0.06}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.cos_tilt_1}{0.1^{+0.4}_{-0.1}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.cos_tilt_2}{0.2^{+0.4}_{-0.2}}
\JSONSetValue{subpop_hyperposteriors.b.sigma.mass_ratio}{0.2^{+0.4}_{-0.1}}
\JSONSetValue{subpop_hyperposteriors.b.rho}{-0.3^{+0.9}_{-0.6}}
\JSONSetValue{subpop_hyperposteriors.c.mu.chi_1}{0.7^{+0.3}_{-0.4}}
\JSONSetValue{subpop_hyperposteriors.c.mu.chi_2}{0.6^{+0.4}_{-0.4}}
\JSONSetValue{subpop_hyperposteriors.c.mu.cos_tilt_1}{0.6^{+0.4}_{-1.1}}
\JSONSetValue{subpop_hyperposteriors.c.mu.cos_tilt_2}{0.2^{+0.8}_{-0.9}}
\JSONSetValue{subpop_hyperposteriors.c.mu.mass_ratio}{0.4^{+0.3}_{-0.4}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.chi_1}{0.4^{+0.4}_{-0.4}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.chi_2}{0.6^{+0.4}_{-0.4}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.cos_tilt_1}{1.1^{+0.8}_{-1.1}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.cos_tilt_2}{1.0^{+1.0}_{-0.8}}
\JSONSetValue{subpop_hyperposteriors.c.sigma.mass_ratio}{0.4^{+0.3}_{-0.3}}
\JSONSetValue{subpop_hyperposteriors.c.rho}{0.0^{+0.9}_{-0.7}}
\JSONSetValue{subpop_ppds.a.chi_1}{0.02^{+0.03}_{-0.02}}
\JSONSetValue{subpop_ppds.a.chi_2}{0.02^{+0.03}_{-0.02}}
\JSONSetValue{subpop_ppds.a.cos_tilt_1}{-0.03^{+0.08}_{-0.09}}
\JSONSetValue{subpop_ppds.a.cos_tilt_2}{-0.01^{+0.10}_{-0.10}}
\JSONSetValue{subpop_ppds.a.mass_ratio}{0.9^{+0.1}_{-0.2}}
\JSONSetValue{subpop_ppds.b.chi_1}{0.16^{+0.10}_{-0.09}}
\JSONSetValue{subpop_ppds.b.chi_2}{0.2^{+0.1}_{-0.2}}
\JSONSetValue{subpop_ppds.b.cos_tilt_1}{0.6^{+0.4}_{-0.6}}
\JSONSetValue{subpop_ppds.b.cos_tilt_2}{0.6^{+0.4}_{-0.6}}
\JSONSetValue{subpop_ppds.b.mass_ratio}{0.9^{+0.1}_{-0.4}}
\JSONSetValue{subpop_ppds.c.chi_1}{0.7^{+0.3}_{-0.5}}
\JSONSetValue{subpop_ppds.c.chi_2}{0.5^{+0.5}_{-0.4}}
\JSONSetValue{subpop_ppds.c.cos_tilt_1}{0.1^{+0.9}_{-0.9}}
\JSONSetValue{subpop_ppds.c.cos_tilt_2}{0.1^{+0.9}_{-0.8}}
\JSONSetValue{subpop_ppds.c.mass_ratio}{0.4^{+0.4}_{-0.4}}
\JSONSetValue{log_bayes_factors.in_favor_of_component_a_being_zero_spin}{6.4^{+0.3}_{-0.5}}

